Enhanced Sub-kpc Scale Star-formation: Results From A JWST Size Analysis of 341 Galaxies At 5<z<14

We present a comprehensive search and analysis of high-redshift galaxies in a suite of nine public JWST extragalactic fields taken in Cycle 1, covering a total effective search area of $\sim358{\rm arcmin^2}$. Through conservative ($8\sigma$) photometric selection, we identify 341 galaxies at $5<z<14$, with 109 having spectroscopic redshift measurements from the literature, including recent JWST NIRSpec observations. Our regression analysis reveals that the rest-frame UV size-stellar mass relation follows $R_{\rm eff}\propto M_*^{0.19\pm0.03}$, similar to that of star-forming galaxies at $z\sim3$, but scaled down in size by $\sim0.7$dex. We find a much slower rate for the average size evolution over the redshift range, $R_{\rm eff}\propto(1+z)^{-0.4\pm0.2}$, than that derived in the literature. A fraction ($\sim13\,\%$) of our sample are marginally resolved even in the NIRCam imaging ($<100$pc), located at $>1.5\,\sigma$ below the derived size-mass slope. These compact sources exhibit a high star formation surface density $\Sigma_{\rm SFR}>10\,M_\odot\,{\rm yr^{-1}\,kpc^{-2}}$, a range in which only $<0.01\,\%$ of the local star-forming galaxy sample is found. For those with available NIRSpec data, no evidence of ongoing supermassive black hole accretion is observed. A potential explanation for the observed high [OIII]-to-Hbeta ratios could be high shock velocities, likely originating within intense star-forming regions characterized by high $\Sigma_{\rm SFR}$. Lastly, we find that the rest-frame UV and optical sizes of our sample are comparable. Our results are consistent with these early galaxies building up their structures inside-out and yet to exhibit the strong color gradient seen at lower redshift.

==> table_mex.tex <==
\begin{deluxetable}{ccc}
    \tablecaption{
    Line ratio measurements used for the MEx diagram.
    }
    \tablehead{
    \colhead{ID} & \colhead{$\log$\,\oiii/\hb} & \colhead{Dist.}\\
    \colhead{} & \colhead{} & \colhead{dex}
    }
    \startdata
glassnircam-5240 & $0.76\pm{0.02}$ & $-0.19\pm{0.02}$\\
glassnircam-7284 & $0.54\pm{0.13}$ & $-0.47\pm{0.13}$\\
glassnircam-7728 & $0.54\pm{0.28}$ & $-0.49\pm{0.28}$\\
glassnircam-9029 & $1.06\pm{0.14}$ & $0.11\pm{0.15}$\\
glassnircam-9694 & $0.77\pm{0.30}$ & $-0.16\pm{0.30}$\\
glassnircam-9701 & $0.43\pm{0.25}$ & $-0.54\pm{0.25}$\\
glassnircam-11854 & $>0.75$ & $-0.73\pm{0.25}$\\
glassnircam-12496 & $0.81\pm{0.13}$ & $-0.11\pm{0.13}$\\
jadesgds-6734 & $0.74\pm{0.07}$ & $-0.13\pm{0.07}$\\
jadesgds-7592 & $>0.21$ & $-0.25\pm{0.07}$\\
jadesgds-8179 & $0.74\pm{0.11}$ & $-0.28\pm{0.11}$\\
jadesgds-8408 & $0.79\pm{0.09}$ & $-0.23\pm{0.09}$\\
jadesgds-9326 & $0.79\pm{0.20}$ & $-0.19\pm{0.20}$\\
jadesgds-10902 & $0.74\pm{0.16}$ & $-0.27\pm{0.16}$\\
jadesgds-11449 & $0.70\pm{0.10}$ & $-0.32\pm{0.10}$\\
jadesgds-11841 & $0.67\pm{0.16}$ & $-0.31\pm{0.16}$\\
jadesgds-12147 & $0.05\pm{0.30}$ & $-0.86\pm{0.30}$\\
jadesgds-14986 & $0.84\pm{0.22}$ & $-0.14\pm{0.22}$\\
jadesgds-16254 & $>0.66$ & $-0.66\pm{0.22}$\\
jadesgds-17941 & $0.69\pm{0.19}$ & $-0.20\pm{0.19}$\\
jadesgds-18169 & $0.75\pm{0.03}$ & $-0.26\pm{0.03}$\\
jadesgds-18204 & $>0.09$ & $-0.05\pm{0.03}$\\
jadesgds-18784 & $0.83\pm{0.34}$ & $-0.05\pm{0.33}$\\
jadesgds-29538 & $0.64\pm{0.07}$ & $-0.35\pm{0.07}$\\
jadesgds-31651 & $0.32\pm{0.19}$ & $-0.10\pm{0.10}$\\
jadesgds-32171 & $0.80\pm{0.14}$ & $-0.12\pm{0.14}$\\
jadesgds-33170 & $0.78\pm{0.05}$ & $-0.23\pm{0.05}$\\
jadesgds-33350 & $0.36\pm{0.12}$ & $-0.65\pm{0.12}$\\
jadesgds-33803 & $1.12\pm{0.22}$ & $0.11\pm{0.22}$\\
jadesgds-34138 & $0.72\pm{0.13}$ & $-0.26\pm{0.13}$\\
jadesgds-35365 & $0.64\pm{0.18}$ & $-0.36\pm{0.18}$\\
ceersnircam1-23089 & $0.81\pm{0.34}$ & $0.07\pm{0.30}$\\
ceersnircam2-1767 & $0.63\pm{0.26}$ & $-0.39\pm{0.26}$\\
ceersnircam2-7005 & $0.70\pm{0.27}$ & $-0.19\pm{0.27}$\\
ceersnircam3-15767 & $0.83\pm{0.15}$ & $-0.17\pm{0.15}$\\
ceersnircam3-18419 & $0.77\pm{0.15}$ & $0.01\pm{0.14}$\\
ceersnircam3-20932 & $0.82\pm{0.05}$ & $-0.05\pm{0.05}$\\
ceersnircam4-9402 & $0.52\pm{0.17}$ & $0.04\pm{0.08}$\\
ceersnircam6-7832 & $0.67\pm{0.12}$ & $-0.28\pm{0.12}$\\
ceersnircam7-18822 & $0.96\pm{0.22}$ & $0.27\pm{0.20}$\\
glassnircam-5260 & $0.89\pm{0.07}$ & $-0.06\pm{0.07}$\\
glassnircam-15395 & $0.90\pm{0.15}$ & $-0.08\pm{0.15}$\\
glassnircam-16993 & $0.98\pm{0.28}$ & $0.22\pm{0.28}$\\
glassnircam-17308 & $>0.84$ & $-0.59\pm{0.29}$\\
glassnircam-17424 & $>0.84$ & $-0.33\pm{0.28}$\\
glassnircam-17751 & $0.88\pm{0.07}$ & $-0.08\pm{0.07}$\\
glassnircam-18185 & $0.65\pm{0.10}$ & $-0.32\pm{0.10}$\\
jadesgds-15413 & $0.76\pm{0.20}$ & $-0.19\pm{0.21}$\\
jadesgds-15571 & $>0.60$ & $-0.50\pm{0.20}$\\
jadesgds-36297 & $0.79\pm{0.14}$ & $-0.22\pm{0.15}$\\
ceersnircam8-9615 & $0.80\pm{0.11}$ & $0.06\pm{0.10}$\\
    \enddata
    \tablecomments{
    $1\,\sigma$ error is quoted. For those with $S/N<3$ in \hb\ flux measurements, $3\,\sigma$ lower limit is shown for the ratio.
    }\label{tab:mex}
    \end{deluxetable}
    
